Unsupervised Instance and Subnetwork Selection for Network Data

Unlike tabular data, features in network data are interconnected within a domain-specific graph. Examples of this setting include gene expression overlaid on a protein interaction network (PPI) and user opinions in a social network. Network data is typically high-dimensional (large number of nodes) and often contains outlier snapshot instances and noise. In addition, it is often non-trivial and time-consuming to annotate instances with global labels (e.g., disease or normal). How can we jointly select discriminative subnetworks and representative instances for network data without supervision? We address these challenges within an unsupervised framework for joint subnetwork and instance selection in network data, called UISS, via a convex self-representation objective. Given an unlabeled network dataset, UISS identifies representative instances while ignoring outliers. It outperforms state-of-the-art baselines on both discriminative subnetwork selection and representative instance selection, achieving up to 10% accuracy improvement on all real-world data sets we use for evaluation. When employed for exploratory analysis in RNA-seq network samples from multiple studies it produces interpretable and informative summaries.

==> tex_SDM/4_problem.tex <==
\section{Problem Formulation}
%we have the data matrix as  $\mathbf{X} = \left [ \mathbf{X}_1,\mathbf{X}_2,...\mathbf{X}_n \right ]^T \in \mathbb{R}^{n\times m}$. 
Given a dataset ${\mathcal{DS}}$ of $n$ unlabeled network instances with $m$ nodes, our goal is to select $p~(p\ll n)$ instances which are representative of the underlying clusters in the dataset when considering the feature values in a connected subgraph subspace of $q~(q\ll m)$ nodes. Intuitively, the above design objective assumes that some instances form (unknown number of) clusters, while others are outliers and do not belong to clusters. Furthermore, this cluster configuration is elucidated within a subspace of connected features (subgraphs of $\mathcal{S}$), whose values are discriminative, i.e. the clusters and outliers are well-separated from each other in this subspace. Note that the above assumptions are very similar to those in supervised learning on networks data~\cite{DIPS,ranu2013mining}, only the discriminative power %of selected subgraphs in our unsupervised setting 
is quantified by cluster and outlier separability as opposed to class separability.  

%To formalize the above intuition we introduce two key variables in our model: (ii) a subgraph and instance selection matrix ${\bf W}\in \mathbb{R}^{m\times n}$, and (ii) an instance association matrix ${\bf Z}\in \mathbb{R}^{n\times n}$.  
%To extract the discriminative information, we take advantage of the cluster information because labels of instances are unavailable.
%Our overall discriminative subgraph and instance selection objective has the following form:
%\begin{equation}\vsa
%    \begin{aligned}
%        &\underset{{\bf W, Z}}{\mathrm{argmin}}  \hspace{0.1CM} \mathcal{J}({\bf W})  +\mathcal{R}({\bf Z,W}),
%    \end{aligned}\vsa
%\end{equation}
%where $\mathcal{J}({\bf W})$ is an instance and subgraph selection function enforcing a sparse, yet truthful approximation of the data matrix, and $\mathcal{R}({\bf Z,W})$ is a discriminative learning function which enforces block-like low-rank structure of the instance association matrix $\bf Z$ in the subspace selected by ${\bf W}$. Next, we discuss the design of the two parts of our objective.
%The selection process and discriminative learning process boost each other within the model by fixing the variable  and $\bf W$ alternatively.
% We will illustrate the details of these functions in the following.
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++

We model the instance and subgraph selection as a function $\mathcal{J}({\bf P,Q})$ which enforces a sparse approximation to the data $\mathbf{X}$. The matrix $\bf P\in \mathbb{R}^{m\times n}$ serves as a selector for features with rows of high norm corresponding to selected features and vice versa. Similarly $\bf Q\in \mathbb{R}^{m\times n}$ serves as an instance selector through the norms of its columns. We approximate the data via a quadratic form of the sum of selector matrices $\left \|\mathbf{X}-\mathbf{X(P+Q)} \mathbf{X}\right \|_{2,1}$.  
%In particular, we employ an  for the data approximation . 
A similar reconstruction function has been considered by recent CUR-based feature selection method for active learning~\cite{Li2018alfs}, however the reconstruction loss in the latter is quantified via the Frobenius norm while we employ the $L_{2,1}$ norm, which is more robust to outliers and noise. We also need to ensure (i) row sparsity for ${\bf P}$ and (ii) column sparsity for ${\bf Q}$ so that they behave as feature and instance selectors. In addition we impose ``smoothness'' on the feature selection with respect to the common graph structure $\mathcal{S}$ to enforce connectivity in the feature space.    
%According to ALFS, important instances and features can be obtained by finding these have the best approximation of the input data via linear combination.
% as $\left \|\mathbf{X}-\mathbf{XW} \mathbf{X}\right \|_F^2$. 
%However, the Frobenius norm based loss function used in ALFS 
%is likely to be dominated by outliers and noise because square error is sensitive to them. 
%To circumvent this problem, 
%The matrix $\bf W$ is responsible for the selection of data rows and columns simultaneously. Directly imposing column and row sparsity on it may be too restrictive and cause oscillation problems during optimization. Instead, we relax this selection as two-component matrix sum $ \mathbf{W}=\mathbf{P}+\mathbf{Q}$,
% P and Q to exploit relationships among columns and rows.
%where $\bf P$ and $\bf Q$ select features and instances, respectively. 
Our selection function $\mathcal{J}({\bf P,Q})$ is as follows:
\begin{equation}\label{Jw1}\vsa
%\footnotesize
        \begin{aligned}
     \mathcal{J}({\bf P},{\bf Q}) &=   \left \|\mathbf{X}-\mathbf{X}(\mathbf{P}+\mathbf{Q}) \mathbf{X}\right \|_{2,1}
        + \lambda_1\left \| \mathbf{P} \right \|_{2,1}+\lambda_2\left \| \mathbf{Q}^T  \right \|_{2,1} \\ &+ \lambda_3\textup{Tr}(\mathbf{P}^T \mathbf{L}\mathbf{P}),
        %& s.t. \hspace{0.1cm} \mathbf{W}=\mathbf{P}+\mathbf{Q}
   \end{aligned} 
\end{equation}
where we impose row sparsity on $\mathbf{P}$ and $\mathbf{Q}^T$ via $L_{2,1}$ regularizers with corresponding weight parameters $\lambda_1$ and $\lambda_2$ to control the number of selected features and instances respectively. %If the $i$-th feature is not important for the reconstruction of ${\mathbf X}$, then the $i$-th row of $\bf P$ will shrink to a zero vector and vice versa. $\mathbf{Q}$'s regularization will behave similarly for column selection. 
The third regularizer $\textup{Tr}(\mathbf{P}^T \mathbf{L}\mathbf{P})$ promotes connectivity in %the aggregate instance graph structure 
$\mathcal{S}$ by penalizing differences in the selection of coefficients associated with connected nodes. To appreciate the above, note that the trace penalizes the sum of squared differences between selection vectors of neighboring nodes due to the properties of the graph Laplacian, i.e.
$
    \textup{Tr}(\mathbf{P}^T \mathbf{L}\mathbf{P})=\frac{1}{2}\sum_i\sum_j\mathbf{M}_{ij}\left \| \mathbf{P}_i-\mathbf{P}_j \right \|_2^2,
$
where $\mathbf{M}_{ij}$ is the weight of the edge between nodes $i$ and $j$ in $\mathcal{S}$.  
% importance of nodes are in the row of P, 
% if ith row is not zeros, mean the ith node is important, vice versa
%$\mathbf{M}_{ij}\left \| \mathbf{P}_i-\mathbf{P}_j \right \|_2^2$. 
%the following
%\begin{equation}\label{J1_W}
%\footnotesize
%    \begin{aligned}
%    &\underset{{\bf P}}{\mathrm{argmin}}\hspace{0.1cm} \mathcal{J}_2({\bf W})=\frac{1}{2}\sum_i\sum_j\mathbf{M}_{ij}\left \| \mathbf{P}_i-\mathbf{P}_j \right \|_2^2
%    =\textup{Tr}(\mathbf{P}^T \mathbf{L}\mathbf{P})\\
%  \end{aligned}  
%\end{equation}
% \begin{equation}\label{J1_W}
% \footnotesize
%     \begin{aligned}
%     &\underset{{\bf P}}{\mathrm{argmin}}\hspace{0.1cm} \mathcal{J}_2({\bf W})=\sum_i\sum_j\mathbf{M}_{ij}\left \| \mathbf{P}\mathbf{X}_i-\mathbf{P}\mathbf{X}_j \right \|_2^2=
%     \textup{Tr}(\mathbf{X}^T\mathbf{P}^T \mathbf{L}\mathbf{P}\mathbf{X})\\
%   \end{aligned}  
% \end{equation}


% where $\bf V= {\bf WX}$ is the reconstruction coefficient matrix.
% More specifically,
% each feature is reconstructed by a linear combination of selected features according to Eq.~\ref{J1_W}.
%In particular, the $i-$th row of ${\bf WX}$ is selected when
% If $i$-th feature  ${\bf X}^i$ is not important, then $i$-th row of $\bf P$ will shrink to zero vector and vice versa. 
% To make the selected nodes well-connected as a subgraph, we enforce the connected nodes to have similar coefficients by minimizing the following
% \begin{equation}\label{J1_W}
% \footnotesize
%     \begin{aligned}
%     &\underset{{\bf P,Q}}{\mathrm{argmin}}\hspace{0.1cm} \mathcal{J}_2({\bf W})=\textup{Tr}(\mathbf{V}^T \mathbf{L}\mathbf{V})\\
%   \end{aligned}  
% \end{equation}
% where $\bf V= {\bf WX}$ is the reconstruction coefficient matrix.
% More specifically,
% each feature is reconstructed by a linear combination of selected features according to Eq.~\ref{J1_W}.
% %In particular, the $i-$th row of ${\bf WX}$ is selected when
% If $i$-th feature  ${\bf X}^i$ is not important, then $i$-th row of $\bf V$ will shrink to zero vector and vice versa. 
%To this end, we define the selection function as $\mathcal{J}({\bf W})=\mathcal{J}_1({\bf W})+\lambda_3\mathcal{J}_2({\bf W})$ for 
%selecting representative instances and subgraphs, which $\lambda_3$ is a balance parameter.



%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++

%\todo{need to explain the following better}
So far our objective ensures instance and connected feature selection by a low-error reconstruction of the data matrix. However, we have not ensured that the selected instances are discriminative, i.e. represent the underlying clusters as opposed to being outliers. We approach the latter by a second part of our objective: the discriminative learning function $\mathcal{R}({\bf Z,P})$. %() should quantify the ability of selected features to distinguish instances from different clusters as well as outliers.
% Therefore, we need to assign cluster labels to instances.
Instead of explicitly modeling cluster memberships and deciding on the number of clusters apriori, we learn a low-rank instance association matrix ${\bf Z}\in \mathbb{R}^{n\times n}$ which ``groups'' similar instances in the feature subspace selected by $\mathbf {P}$: %We define the discriminative learning function as follows:  
\begin{equation}\label{RZ1}
    \begin{aligned}
         \mathcal{R}({\bf Z,P})=\alpha_1\left \| \mathbf{X}\mathbf{P}-\mathbf{Z} \right \|_{2,1}+\alpha_2 \left \| \mathbf{Z} \right \|_*,
    \end{aligned}
\end{equation}
where $\alpha_1$ and $\alpha_2$ are balance parameters. The first part of $\mathcal{R}({\bf Z,P})$ ensures that the projection of instances $\mathbf{X}_i \mathbf{P}^j$ onto feature selector vectors in $\bf P$ is aligned with the instance association matrix $\mathbf{Z}$, while in the second part we enforce a low rank on ${\bf Z}$ by the nuclear norm which is a widely-adopted relaxation for rank minimization~\cite{recht2008necessary}. 

Another way to interpret $\mathcal{R}({\bf Z,P})$ is through the lens of %recent work on 
multi-label learning~\cite{xu2014learning}, where the goal is to train a multi-label predictor by explicitly modeling label correlations. In our case, we assume that each instance is labeled with a unique label (i.e. the label matrix is the identity $\mathbf{I}$) and we are learning the association of labels (instances) through $\mathbf{Z}$. Notable difference from the above is that we are working in an unsupervised setting and that we impose $L_{2,1}$ norm instead of the more common Frobenius norm in order to minimize the effect of outlier instances. 

%One can also interpret  $\left \|\mathbf{X}\mathbf{P}-\mathbf{Z} \right \|_{2,1}$ as a label learning objective in which all instances are assigned an individual labels \todo{citation:} \textcolor{blue}{This is my own original idea. This is my contribution for discriminative learning when no lables...} . 

%$\mathbf{X}\mathbf{P}-\mathbf{Y}\mathbf{Z}$
%Instead of learning pseudo labels for instances directly, which is commonly used in related unsupervised learning methods, we assume that each instance has a unique label, i.e. the label matrix  ${\bf Y}\in \mathbb{R}^{n\times n}$ of instances is an identity matrix. 
%Clearly, these instances are not independent of each other, so are their labels.



%\todo{what does the following mean?}Such a label representation provides a rich semantic information. 
%With the label information, our unsupervised 
%discriminative feature learning problem is converted into a supervised problem, and we aim to solve the following optimization problem:
%By adopting the least square loss, we can 
% We now propose a new solution as follows
%learn such a correlation matrix to model the cluster information implicitly.
%To address the uncertainty of latent cluster numbers, we propose the following optimization problem
 %The cost function applies L21 loss to enhance the robustness to noise and outliers.
%The ${\bf P}_i$ will shrink to zero if $i^{th}$ feature is less correlated to the label $\bf Z$. 
%The second term is to enforce the correlation matrix has a small rank
%ue to the fact that these labels from the same class are strongly correlated and  differentiated from those from different classes.
% among labels to be small because instances often originate from a few classes in real-world data. , 

%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++
%  ++++++++++++++++++++++++++++++++++++++++++


Combining $\mathcal{J}({\bf P,Q})$ and $\mathcal{R}({\bf Z,P})$,  
%and discriminative learning function $\mathcal{G}({\bf W})$, 
% the most representative instances and discriminative subgraphs will be found
% Combining $\mathcal{J}({\bf W})$, $\mathcal{R}({\bf Z})$ and $\mathcal{G}({\bf W})$,
we get the following objective:
\begin{equation}\label{objective}
%\footnotesize
        \begin{aligned}
    &\underset{{\bf P,Q,Z}}{\mathrm{argmin}} \left \|\mathbf{X}-\mathbf{X(P+Q)} \mathbf{X}\right \|_{2,1}
        + \lambda_1\left \| \mathbf{P} \right \|_{2,1}+\lambda_2\left \| \mathbf{Q}^T  \right \|_{2,1}\\
        &+ \lambda_3 \textup{Tr}(\mathbf{P}^T \mathbf{L}\mathbf{P})
        + \alpha_1\left \| \mathbf{X}\mathbf{P}-\mathbf{Z} \right \|_{2,1}+\alpha_2 \left \| \mathbf{Z} \right \|_*,\\
        %& s.t. \mathbf{W}=\mathbf{P}+\mathbf{Q}
        %\left\{\begin{matrix}
%         & \mathbf{W}=\mathbf{P}+\mathbf{Q} \\
% &\mathbf{Z}_{i,j}\geq 0, & \text{for all } i,j\\
%  %\sum_{j} \mathbf{Z}_{i,j} = 1, &\text{ for  all } i \\ 
%\end{matrix}\right.
   \end{aligned}  
\end{equation}
which enforces all our design goals: joint (i) connected feature selection encoded in $\mathbf{P}$, and (ii) discriminative (non-outlier) instance selection, where selected instances are encoded in $\mathbf{Q}$ and discriminative power is achieved by imposing a low-rank structure on $\mathbf{Z}$. It is important to note that our learned model also provides structural interpretation of the solution in two ways: (i) it learns discriminative connected subgraph regions in $\mathcal{S}$ which may correspond to protein complexes in PPIs, functional brain subnetworks, etc.; and (ii) it learns a relational structure among instances in $\mathbf{Z}$.%, which can be used for clustering, outlier detection and for active learning.     
